Learning to Compose Visual Relations

The visual world around us can be described as a structured set of objects and their associated relations. An image of a room may be conjured given only the description of the underlying objects and their associated relations. While there has been significant work on designing deep neural networks which may compose individual objects together, less work has been done on composing the individual relations between objects. A principal difficulty is that while the placement of objects is mutually independent, their relations are entangled and dependent on each other. To circumvent this issue, existing works primarily compose relations by utilizing a holistic encoder, in the form of text or graphs. In this work, we instead propose to represent each relation as an unnormalized density (an energy-based model), enabling us to compose separate relations in a factorized manner. We show that such a factorized decomposition allows the model to both generate and edit scenes that have multiple sets of relations more faithfully. We further show that decomposition enables our model to effectively understand the underlying relational scene structure. Project page at: https://composevisualrelations.github.io/.

==> algorithms/algorithm.tex <==
\begin{figure}[t!]
\begin{center}
\includegraphics[width=1\textwidth]{figs/fig-image/algorithms.png}
\end{center}
\vspace{-10pt}
\caption{\small Algorithms for training and testing (\ie image generation, image editing
and image-text retrieval).}
\label{fig:caption_predcitions}
\vspace{-15pt}
\end{figure}

==> figs/fig-text/generalization.tex <==
\begin{figure}[t!]
\begin{center}
\includegraphics[width=1\textwidth]{figs/fig-image/generalization.pdf}
\end{center}
\caption{\small Quantitative evaluation of relation generalization of our EBMs by ranking
different captions.}
\label{fig:caption_predcitions}
\vspace{-10pt}
\end{figure}

==> figs/fig-text/image_generation_block_1_relations.tex <==
\begin{figure}[t]
\begin{center}
\includegraphics[width=0.75\textwidth]{figs/fig-image/image_generation_block_1_relations.pdf}
\end{center}
\vspace{-10pt}
\caption{\small Examples of image generation on real-world block scenes based on a single scene relation. We compare
our main method (Learned Embed) with baselines, such as StyleGAN2 (CLIP), Ours (CLIP) (Sentence) which uses CLIP as the only text encoder to encoder relational scene descriptions of one object relation.}
\label{fig:image_generation_block_1}
\vspace{-10pt}
\end{figure}




==> figs/fig-text/image_generation_block_2_relations.tex <==
\begin{figure}[t]
\begin{center}
\includegraphics[width=\textwidth]{figs/fig-image/image_generation_block_2_relations.pdf}
\end{center}
\vspace{-10pt}
\caption{\small Examples of image generation on real-world block scenes based on two scene relations. Note that
given relational scene descriptions are out of the training distribution.}
\label{fig:image_generation_block_2}
\vspace{-10pt}
\end{figure}




==> figs/fig-text/image_generation_block_3_relations.tex <==
\begin{figure}[t]
\begin{center}
\includegraphics[width=0.75\textwidth]{figs/fig-image/image_generation_block_3_relations.pdf}
\end{center}
\vspace{-10pt}
\caption{\small Examples of image generation on real-world block scenes based on three scene relations. 
Given relational scene descriptions are also out of the training distribution.}
\label{fig:image_generation_block_3}
\vspace{-10pt}
\end{figure}




==> tables/clevr_human_evaluation.tex <==
\begin{wraptable}{r}{.525\linewidth}
\vspace{-15pt}
    \small
    \caption{\small Quantitative evaluation of \textbf{relational similarity} of objects on Clevr dataset. It measures a graph similarity for constructed scene graphs of generated and real images.}
    \vspace{-5pt}
    \label{table:human_eval}
    \begin{tabular}{l|ccc}
        \toprule
        \bf Model & \multicolumn{3}{c}{\bf Matching Score (\%)} \\
        \midrule
        & 1R Acc & 2R Acc & 3R Acc \\
        \midrule
        StyleGAN2 & 22.37 & 19.75 & 17.13 \\
        \cmidrule{1-4}
        StyleGAN2 (CLIP) & 37.50 & 28.62 & 28.75 \\
        \cmidrule{1-4}
        Ours (Learned Emb) & \bf 50.77 & \bf 36.87 & \bf 42.50 \\
        \bottomrule
    \end{tabular}
\vspace{-10pt}
\end{wraptable}

==> tables/generalization_classification.tex <==
\begin{table}[t]
    \centering
    \small
    \caption{Quantitative evaluation of the image binary classifier. 1R, 2R and 3R indicate one, two and three relations nesting respectively. Dataset for \textbf{Classification} contains default CLEVR objects, and
    dataset for \textbf{Generalization} contains boot, toy and truck objects.}
    \label{table:generalization_classification}
    \begin{tabular}{c|ccc|ccc}
        \toprule
        \bf Model & \multicolumn{3}{c|}{\bf Classification (\%)} & \multicolumn{3}{c}{\bf Generalization (\%)}\\
        \midrule
        & 1R Acc & 2R Acc & 3R Acc & 1R Acc & 2R Acc & 3R Acc \\
        \midrule
        CLIP (Pretrained) & 3.67 & 0.67 & 0 & 2.33 & 0 & 0 \\
        \cmidrule{1-7}
        CLIP (Fine-tuned) (CLIP) & 31.67 & 14.37 & 8.00 & 6.67 & 0 & 0 \\
        \cmidrule{1-7}
        Ours (CLIP) &  &  &  & 0.67 & 0 &  \\
        \cmidrule{1-7}
        Ours (Learned Embedding) & 11.67  & 3.33 &  & 7.00 & 3.30 & 0  \\
        \bottomrule
    \end{tabular} 
\end{table}









% \begin{table}[t!]
%     \centering
%     \small
%     \caption{Quantitative evaluation of the image binary classifier. 1R, 2R and 3R indicate one, two and three relations nesting respectively. Dataset for \textbf{Classification} contains default CLEVR objects, and
%     dataset for \textbf{Generalization} contains boot, toy and truck objects.}
%     \label{table:generalization_classification}
%     \begin{tabular}{c|ccc|ccc}
%         \toprule
%         \bf Model & \multicolumn{3}{c|}{\bf Classification (\%)} & \multicolumn{3}{c}{\bf Generalization (\%)}\\
%         \midrule
%         & 1R Acc & 2R Acc & 3R Acc & 1R Acc & 2R Acc & 3R Acc \\
%         \midrule
%         Classifier & 97.72 & 95.56 & 93.68 & 78.60 & 66.30 & 58.58 \\
%         \cmidrule{1-7}
%         CLIP (Pretrained) & 28.30 & 11.84 & 5.52 & 36.06 & 14.78 & 7.34 \\
%         \cmidrule{1-7}
%         CLIP (Fine-tuned) (CLIP) & 81.88 & 69.16 & 60.48 & 56.80 & 35.72 & 24.12 \\
%         \cmidrule{1-7}
%         Ours (CLIP) & \bf 99.90 & \bf 99.88 & \bf 99.80  & \bf 99.95 & \bf 99.88 & \bf 99.88\\
%         \cmidrule{1-7}
%         Ours (Learned Embedding) & 98.00 & 97.08 & 96.45 & 91.70 & 87.25 & 84.45 \\
%         \bottomrule
%     \end{tabular} 
% \end{table}

% \begin{table}
%     \centering
%     \small
%     \label{fid:generalization}
%     \begin{tabular}{|c|c|c|c|c|c|c|c|c|}
%         \toprule
%         & & \multicolumn{3}{c|}{Classification} & \multicolumn{3}{c|}{Generalization} \\
%         \midrule
%         Dataset & Model & 1R & 2R & 3R & 1R & 2R & 3R \\
%         \midrule
%         \multirow{6}{*}{Clevr} & Classifier & 0.977 & 0.956 & 0.937 & 0.786 & 0.663 & 0.586 \\
%                                  \cmidrule{2-8}
%                                  & CLIP (Pretrained) & 0.283 & 0.118 & 0.055 & 0.361 & 0.148 & 0.073 \\
%                                  \cmidrule{2-8}
%                                  & CLIP (Fine-tuned) & 0.819 & 0.692 & 0.605 & 0.568 & 0.357 & 0.241 \\
%                                  \cmidrule{2-8}
%                                  & Ours (CLIP) & 1.000 & 1.000 & 1.000 & 1.000 & 1.000 & 1.000 \\
%                                  \cmidrule{2-8}
%                                  & Ours (Learned Embedding) & 0.968 & 0.956 & 0.948 & 0.871 & 0.816 & 0.782 \\
%         \bottomrule
%     \end{tabular}
%     \bigskip
%     \caption{Quantitative evaluation of both Clevr dataset and generalization dataset.}
% \end{table}

==> tables/image_generation_editing_quality.tex <==
\begin{table}[t]
    \centering
    \small
    \caption{Quantitative evaluation of image generation on both Clevr and iGibson dataset using
    EBMs and variants of StyleGAN2 (ADA) \citep{karras2020training} where StyleGAN2 is unconditional
    generates images by running latent optimization to satisified a separated trained classifier, 
    and StyleGAN2 (CLIP) conditions on text embeddings from a pretrained encoder of CLIP model \citep{radford2021learning}.
    Ours (CLIP) encodes object description using CLIP's pretrained text encoder, while relation is learned through the EBM. Ours (Learned Embedding) learns embeddings of all attributes.}
    \label{table:image_generation_editing_quality}
    \begin{tabular}{c|c|cc|cc|cc}
        \toprule
         \bf Dataset  & \bf Model  & \multicolumn{2}{c|}{\bf 1R Acc} & \multicolumn{2}{c|}{\bf 2R Acc} & \multicolumn{2}{c}{\bf 3R Acc} \\
        \midrule
        & &  FID $\downarrow$ & KID $\downarrow$ & FID $\downarrow$ & KID $\downarrow$ & FID $\downarrow$ & KID $\downarrow$ \\
        \midrule
        \multirow{5}{*}{Clevr} & StyleGAN2 & 56.68 & 0.0330 & 65.05 & \bf 0.0347 & 67.53 & \bf 0.0345 \\
                                 \cmidrule{2-8}
                                %  & StyleGAN2 (CLIP) & \textbf{19.97} & \textbf{0.0141} & \textbf{31.22} & \textbf{0.0234} & \textbf{31.70} & \textbf{0.0238} \\
                                 \cmidrule{2-8}
                                 & Ours (CLIP) & \bf 37.95 & \bf 0.0311 & \bf 49.11 & 0.0436 & \bf 50.95 & 0.0447\\
                                 \cmidrule{2-8}
                                 & Ours (Learned Embedding) & 42.38 & 0.0362 & 55.15 & 0.0487 & 57.94 & 0.0509\\
        \midrule
        \multirow{5}{*}{iGibson} 
        & StyleGAN2 & 134.42 & 0.1811 & 127.48 & 0.1751 & 121.47 & 0.1667 \\
                                 \cmidrule{2-8}
                                %  & StyleGAN2 (CLIP) & \textbf{103.60} & \textbf{0.1519} & \textbf{109.96} & 0.1628 & \textbf{114.50} & 0.1690\\
                                 \cmidrule{2-8}
                                 & Ours (CLIP) & \bf 118.90 & \bf 0.1621 & \bf 117.34 & \textbf{0.1601} & \bf 117.55 & \textbf{0.1605}\\
                                 \cmidrule{2-8}
                                 & Ours (Learned Embedding) & 146.22 & 0.2125 & 147.32 & 0.2178 & 149.39 & 0.2215 \\
        \bottomrule
    \end{tabular}
\end{table}

==> text/checklist.tex <==

\section*{Checklist}

% %%% BEGIN INSTRUCTIONS %%%
% The checklist follows the references.  Please
% read the checklist guidelines carefully for information on how to answer these
% questions.  For each question, change the default \answerTODO{} to \answerYes{},
% \answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
% justification to your answer}, either by referencing the appropriate section of
% your paper or providing a brief inline description.  For example:
% \begin{itemize}
%   \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
%   \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
%   \item Did you include the license to the code and datasets? \answerNA{}
% \end{itemize}
% Please do not modify the questions and only use the provided macros for your
% answers.  Note that the Checklist section does not count towards the page
% limit.  In your paper, please delete this instructions block and only keep the
% Checklist section heading above along with the questions/answers below.
% %%% END INSTRUCTIONS %%%

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{See \sect{sect:conclusion}.}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerYes{See \sect{sect:conclusion}.}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerNA{}
	\item Did you include complete proofs of all theoretical results?
    \answerNA{}
\end{enumerate}

\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{See supplemental material.}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{See supplemental material.}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerNA{}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{See supplemental material.}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{}
  \item Did you mention the license of the assets?
    \answerYes{}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerYes{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerYes{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerYes{}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}

\end{enumerate}



==> text/societal_impact.tex <==
\section{Societal Impact}

One main potential negative societal impact of our work is that training a neural network
often triggers a long usage of electricity. Empirically, neural networks usually require
to find a suitable set of hyperparameters to perform reasonably, and training EBMs often
requires a similar procedure. This may potentially cause some intermediate waster of resources that
could negatively impact our environments.
